Design, Evaluation and Analysis of Combinatorial Optimization Heuristic Algorithms

Combinatorial optimization is widely applied in a number of areas nowadays. Unfortunately, many combinatorial optimization problems are NP-hard which usually means that they are unsolvable in practice. However, it is often unnecessary to have an exact solution. In this case one may use heuristic approach to obtain a near-optimal solution in some reasonable time. We focus on two combinatorial optimization problems, namely the Generalized Traveling Salesman Problem and the Multidimensional Assignment Problem. The first problem is an important generalization of the Traveling Salesman Problem; the second one is a generalization of the Assignment Problem for an arbitrary number of dimensions. Both problems are NP-hard and have hosts of applications. In this work, we discuss different aspects of heuristics design and evaluation. A broad spectrum of related subjects, covered in this research, includes test bed generation and analysis, implementation and performance issues, local search neighborhoods and efficient exploration algorithms, metaheuristics design and population sizing in memetic algorithm. The most important results are obtained in the areas of local search and memetic algorithms for the considered problems. In both cases we have significantly advanced the existing knowledge on the local search neighborhoods and algorithms by systematizing and improving the previous results. We have proposed a number of efficient heuristics which dominate the existing algorithms in a wide range of time/quality requirements. Several new approaches, introduced in our memetic algorithms, make them the state-of-the-art metaheuristics for the corresponding problems. Population sizing is one of the most promising among these approaches; it is expected to be applicable to virtually any memetic algorithm.

==> case_problems.tex <==
\chapter{Case study problems}
\label{sec:case_problems}

We start this work from explanation of our case problems.  We have selected the Generalized Traveling Salesman Problem and the Multidimensional Assignment Problem for this purpose.  Both problems are known to be important NP-hard optimization problems yet studied not enough.

\section{Generalized Traveling Salesman Problem}
\label{sec:gtsp}

The \emph{generalized traveling salesman problem} (GTSP) is defined as follows.  We are given a weighted complete directed or undirected graph $G$ and a partition $V = V_1 \cup V_2 \cup \ldots \cup V_M$ of its vertices; the subsets $V_i$ are called {\em clusters}.  The objective is to find a minimum weight cycle containing exactly one vertex from each cluster.  

There are many publications on GTSP (see, e.g., the surveys~\cite{Fischetti2002,Gutin2003} and the references there) and the problem has many applications in warehouse order picking with multiple stock locations, sequencing computer files, postal routing, airport selection and routing for courier planes and some others, see, e.g., \citep{Fischetti1995,Fischetti1997,Laporte1996,Noon1991} and references there.

The problem is NP-hard, since the \emph{Traveling Salesman Problem} (TSP) is a special case of GTSP when $|V_i| = 1$ for each $i$.  GTSP is trickier than TSP in the following sense: it is an NP-hard problem to find a minimum weight collection of vertex-disjoint cycles such that each cluster has only one vertex in the collection (and the claim holds even when each cluster has just two vertices)~\cite{Gutin2003a}.  Compare it with the well-known fact that a minimum weight collection of vertex-disjoint cycles in a weighted complete digraph can be found in polynomial time~\cite{Gutin2007}.

We call GTSP and TSP \emph{symmetric} if the complete graph $G$ is undirected and \emph{asymmetric} if $G$ is directed.  Often instead of the term weight we use the term \emph{length}.



\subsection{Existing Approaches}
\label{sec:gtsp_existing_approaches}

Various approaches to GTSP have been studied.  There are exact algorithms such as branch-and-bound and branch-and-cut algorithms in~\cite{Fischetti1997}. While exact algorithms are very important, they are unreliable with respect to their running time that can easily reach many hours or even days. For example, the well-known TSP solver \textsc{Concorde}~\cite{Applegate2005} can easily solve some TSP instances with
several thousand cities, but it could not solve several asymmetric instances with 316 cities within the time limit of $10^4$ sec. (in fact, it appears it would fail even if significantly much more time was allowed)~\cite{Fischetti1997}.

Several researchers use transformations of GTSP to TSP~\cite{Ben-Arieh2003,Laporte1999,Noon1993} as there exists a large variety of exact and heuristic algorithms for the TSP, see, e.g.,~\cite{Gutin2007,Lawler1985}.  However, while the known transformations normally allow to produce GTSP optimal solutions from the obtained optimal TSP tours, all known transformations do not preserve suboptimal solutions.  Moreover, conversions of near-optimal TSP tours may well result in infeasible GTSP solutions.  Thus, the transformation do not allow us to obtain quickly approximate GTSP solutions and there is a necessity for specific GTSP heuristics. Not every TSP heuristic can be extended to GTSP; for example, so-called subtour patching heuristics often used for the Asymmetric TSP, see, e.g.,~\cite{Johnson2002a}, cannot be extended to GTSP due to the above mentioned NP-hardness result from~\cite{Gutin2003a}.

It appears that the only metaheuristic algorithms that can compete with Lin-Kirnighan-based local search for TSP are memetic algorithms~\cite{Hart2004,Moscato1999} that combine powers of genetic and local search algorithms~\cite{Johnson2002,Tsai2004}.  Thus, it is no coincidence that the latest studies in the area of GTSP explore the memetic algorithm approach~\cite{Bontoux2009,GK_GTSP_GA_2008,Silberholz2007,Snyder2000}.








\section{Multidimensional Assignment Problem}
\label{sec:map}

The \emph{Multidimensional Assignment Problem} (MAP) (abbreviated $s$-AP in the case of $s$ dimensions, also called \emph{(axial) Multi Index Assignment Problem}, MIAP, \citep{Bandelt2004,Pardalos2000}) is a well-known optimization problem.  It is an extension of the \emph{Assignment Problem} (AP), which is exactly the two dimensional case of MAP\@.  While AP can be solved in the polynomial time \citep{Kuhn1955}, $s$-AP for every $s \ge 3$ is NP-hard \citep{Garey1979} and inapproximable \citep{Burkard1996}\footnote{Burkard et al.\ show it for a special case of 3-AP and since 3-AP is a special case of $s$-AP the result can be extended to the general MAP.}\@.

The most studied case of MAP is the case of three dimensions \citep{Aiex2005,Andrijich2001,Balas1991,Crama1992,Huang2006,Spieksma2000} though the problem has a host of applications for higher numbers of dimensions, e.g., in matching information from several sensors (data association problem), which arises in plane tracking \citep{Murphey1998,Pardalos2000b}, computer vision \citep{Veenman2003} and some other applications \citep{Andrijich2001,Bandelt2004,Burkard1999}, in routing in meshes \citep{Bandelt2004}, tracking elementary particles \citep{Pusztaszeri1996}, solving systems of polynomial equations \citep{Bekker2005}, image recognition \citep{Grundel2004}, resource allocation \citep{Grundel2004}, etc.

For a fixed $s \ge 2$, the problem $s$-AP is stated as follows.  Let $X_1 = X_2 = \ldots = X_s = \{1, 2, \ldots, n \}$; we will consider only vectors that belong to the Cartesian product $X = X_1 \times X_2 \times \ldots \times X_s$.  Each vector $e \in X$ is assigned a non-negative weight $w(e)$.  For a vector $e \in X$, the component $e_j$ denotes its $j$th coordinate, i.e., $e_j \in X_j$.  A collection $A$ of $t \le n$ vectors $A^1, A^2, \ldots, A^t$ is a \emph{(feasible) partial assignment} if $A^i_j \neq A^k_j$ holds for each $i \neq k$ and $j \in \{ 1, 2, \ldots, s \}$.  The \emph{weight} of a partial assignment $A$ is $w(A) = \sum_{i=1}^t w(A^i)$.  A partial assignment with $n$ vectors is called \emph{assignment}.  The objective of $s$-AP is to find an assignment of minimal weight.  

A graph formulation of the problem (see Fig.~\ref{fig:map_example}) is as follows.  Having an $s$-partite graph $G$ with parts $X_1$, $X_2$, \ldots, $X_s$, where $|X_i| = n$, find a set of $n$ disjoint cliques in $G$ of the minimal total weight if every clique $Q$ in $G$ is assigned a weight $w(Q)$ (note that in the general case $w(Q)$ is not simply a function of the edges of $Q$).
\begin{figure}[ht]
\centerline{
\xymatrix@-1pc@R=20pt@C=50pt{
		*++[o][F-]{1} \ar@{.}[ddr] 
	&	*++[o][F-]{1} \ar@{-}[r] 
	&	*++[o][F-]{1}
\\
		*++[o][F-]{2} \ar@{-}[ur] 
	&	*++[o][F-]{2} \ar@{~}[dr] 
	&	*++[o][F-]{2}
\\
		*++[o][F-]{3} \ar@{~}[ur] 
	&	*++[o][F-]{3} \ar@{.}[dr] 
	&	*++[o][F-]{3}
\\
		*++[o][F-]{4} \ar@{-}[r] 
	&	*++[o][F-]{4} \ar@{-}[uur] 
	&	*++[o][F-]{4}
\\
	X_1 & X_2 & X_3
}
}
\caption{An example of an assignment for a problem with $s = 3$ and $n = 4$.  This assignment contains the following vectors: (1, 3, 4), (2, 1, 1), (3, 2, 3) and (4, 4, 2). }
\label{fig:map_example}
\end{figure}

An integer programming formulation of the problem can be found in \citep{GK_MAP_LS_2010}.

% is as follows:
%$$
%\min \sum_{i_1 \in X_1, \ldots, i_s \in X_s} w(i_1 \ldots i_s) \cdot x_{i_1 \ldots i_s}
%$$
%subject to
%$$
%\sum_{i_2 \in X_2, \ldots, i_s \in X_s} x_{i_1 \ldots i_s} = 1 \qquad {\forall i_1 \in X_1} \mbox{ ,}
%$$ bnnnnnnnnnnnnnnnn 
%$$
%\ldots
%$$
%$$
%\sum_{i_1 \in X_1, \ldots, i_{s-1} \in X_{s-1}} x_{i_1 \ldots i_s} = 1 \qquad {\forall i_s \in X_s} \mbox{ ,}
%$$
%where $x_{i_1 \ldots i_s} \in \{ 0, 1 \}$ for all $i_1$, \ldots, $i_s$ and $|X_1| = \ldots = |X_s| = n$.

A \emph{permutation form} of the assignment which is sometimes very convenient.  Let $\pi_1, \pi_2, \ldots, \pi_s$ be permutations of $X_1, X_2, \ldots, X_s$, respectively.  Then $\pi_1 \pi_2 \ldots \pi_s$ is an assignment of weight $\sum_{i=1}^n w(\pi_1(i) \pi_2(i) \ldots \pi_s(i))$.  It is obvious that some permutation, say the first one, may be fixed without any loss of generality: $\pi_1 = 1_n$, where $1_n$ is the identity permutation of $n$ elements.  Then the objective of the problem is as follows:
$$
\min_{\pi_2, \ldots, \pi_s} \sum_{i=1}^n w(i \pi_2(i) \ldots \pi_s(i))
$$
and it becomes clear that there exist $n!^{s-1}$ feasible assignments and the fastest known algorithm to find an optimal assignment takes $O(n!^{s-2} n^3)$ operations.  Indeed, without loss of generality set $\pi_1 = 1_n$ and for every combination of $\pi_2, \pi_3, \ldots, \pi_{s-1}$ find the optimal $\pi_s$ by solving corresponding AP in $O(n^3)$.

Thereby, MAP is very hard; it has $n^s$ values in the weight matrix, there are $n!^{s-1}$ feasible assignments and the best known algorithm takes $O(n!^{s-2} n^3)$ operations.  Compare it, e.g., with the Travelling Salesman Problem which has only $n^2$ weights, $(n - 1)!$ possible tours and which can be solved in $O(n^2 \cdot 2^n)$ time \citep{Held1962}.

Finally, an integer programming formulation of the problem is as follows.
$$
\min \sum_{i_1 \in X_1, \ldots, i_s \in X_s} w(i_1 \ldots i_s) \cdot x_{i_1 \ldots i_s}
$$
subject to
$$
\sum_{i_2 \in X_2, \ldots, i_s \in X_s} x_{i_1 \ldots i_s} = 1 \qquad {\forall i_1 \in X_1} \,,
$$
$$
\ldots
$$
$$
\sum_{i_1 \in X_1, \ldots, i_{s-1} \in X_{s-1}} x_{i_1 \ldots i_s} = 1 \qquad {\forall i_s \in X_s} \,,
$$
where $x_{i_1 \ldots i_s} \in \{ 0, 1 \}$ for all $i_1$, \ldots, $i_s$ and $|X_1| = \ldots = |X_s| = n$.

The problem described above is called \emph{balanced} \citep{Clemons2004}.  Sometimes MAP is formulated in a more general way if $|X_1| = n_1$, $|X_2| = n_2$, \ldots, $|X_s| = n_s$ and the requirement $n_1 = n_2 = \ldots = n_s$ is omitted.  However this case can be easily transformed into the balanced problem by complementing the weight matrix to an $n \times n \times \ldots \times n$ matrix with zeros, where $n = \max_i n_i$.

In what follows we assume that the number of dimensions $s$ is a small fixed constant while the size $n$ can be arbitrary large.  This corresponds to the real applications (see above) and also follows from the previous research, see, e.g., \cite{Bekker2005,Pusztaszeri1996,Robertson2001}.



\subsection{Existing Approaches}
\label{sec:map_existing_approaches}

MAP was studied by many researchers.  Several special cases of the problem were intensively studied in the literature (see \cite{Kuroki2007} and references there) but only for a few classes of them polynomial time exact algorithms were found, see, e.g., \cite{Burkard1996a,Burkard1996,Isler2005}.  In many cases MAP remains hard to solve \citep{Burkard1996,Crama1992,Kuroki2007,Spieksma1996}.  For example, if there are three sets of points of size $n$ on a Euclidean plain and the objective is to find $n$ triples, every triple has a point in each set, such that the total circumference or area of the corresponding triangles is minimal, the corresponding 3-APs are still NP-hard \citep{Spieksma1996}.  Apart from proving NP-hardness, researches studied asymptotic properties of some special instance families \citep{Grundel2004,GK_Some_Theory}.

As regards the solution methods, there exist several exact and approximation algorithms~\citep{Balas1991,Crama1992,Kuroki2007,Pasiliao2005,Pierskalla1968} and a number of heuristics including construction heuristics~\cite{Balas1991,Gutin2008,GK_MAP_Construction,Oliveira2004}, greedy randomized adaptive search procedures~\cite{Aiex2005,Murphey1998,Oliveira2004,Robertson2001} (including several concurrent implementations, see, e.g.,~\cite{Aiex2005,Oliveira2004}) and a host of local search procedures~\cite{Aiex2005,Balas1991,Bandelt2004,Burkard1996,Clemons2004,GK_MAP_LS_2010,Huang2006,Oliveira2004,Robertson2001}.

%Construction heuristics give us flexibility to generate a solution with some certain quality requirements (in case of approximation algorithms one can even get some quality guarantee).  Using a local search algorithm, one is able to further improve the solution.  However, a standard local search can optimize the solution only to a local minimum and no further improvements are available after that.  Variable Neighborhood Descend (see, e.g., \cite{Talbi2009}) yields more powerful algorithms \citep{GK_MAP_LS_2010} which, though, still have properties of local search.  In order to improve the solution even more one should use more powerful metaheuristics.

%Metaheuristic is a template for solving hard optimization problems.  A metaheuristic itself is not specific for a certain problem but it may use some subroutines like local search which are designed for a particular problem.  Most of the metaheuristics are inspired by real world processes like genetic, ant colony or simulated annealing algorithms \cite{Talbi2009}.

%Since MAP is a hard combinatorial optimization problem, which often cannot be solved exactly in any reasonable time even for moderate size instances, it is natural to use metaheuristics to solve it.  
Two metaheuristics were proposed for MAP in the literature, namely a simulated annealing procedure \citep{Clemons2004} and a memetic algorithm \citep{Huang2006}.



